Dynamic Role Authorization in Multiparty Conversations

Protocol specifications often identify the roles involved in communications. In multiparty protocols that involve task delegation it is often useful to consider settings in which different sites may act on behalf of a single role. It is then crucial to control the roles that the different parties are authorized to represent, including the case in which role authorizations are determined only at runtime. Building on previous work on conversation types with flexible role assignment, here we report initial results on a typed framework for the analysis of multiparty communications with dynamic role authorization and delegation. In the underlying process model, communication prefixes are annotated with role authorizations and authorizations can be passed around. We extend the conversation type system so as to statically distinguish processes that never incur in authorization errors. The proposed static discipline guarantees that processes are always authorized to communicate on behalf of an intended role, also covering the case in which authorizations are dynamically passed around in messages.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Marco Carbone (Ed.): Third Workshop on\\
Behavioural Types (BEAT 2014)\\
EPTCS 162, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.162.1}{10.4204/EPTCS.162.1}}

